ALLaVA: Harnessing GPT4V-Synthesized Data for Lite Vision-Language Models

Large vision-language models (LVLMs) have shown premise in a broad range of vision-language tasks with their strong reasoning and generalization capabilities. However, they require considerable computational resources for training and deployment. This study aims to bridge the performance gap between traditional-scale LVLMs and resource-friendly lite versions by adopting high-quality training data. To this end, we propose a comprehensive pipeline for generating a synthetic dataset. The key idea is to leverage strong proprietary models to generate (i) fine-grained image annotations for vision-language alignment and (ii) complex reasoning visual question-answering pairs for visual instruction fine-tuning, yielding 1.3M samples in total. We train a series of lite VLMs on the synthetic dataset and experimental results demonstrate the effectiveness of the proposed scheme, where they achieve competitive performance on 17 benchmarks among 4B LVLMs, and even perform on par with 7B/13B-scale models on various benchmarks. This work highlights the feasibility of adopting high-quality data in crafting more efficient LVLMs. We name our dataset \textit{ALLaVA}, and open-source it to research community for developing better resource-efficient LVLMs for wider usage.

==> draft.tex <==
\subsection{Qualitative Results}



\begin{table*}[!t]
% \vspace{-10pt}
\scriptsize
\centering
% \begin{tabular}{llcp{5cm}l}
\begin{tabular}{p{1.8cm}p{9cm}}
\toprule
\multicolumn{2}{l}{\textbf{Example 1: humor comprehension}}  \\
\midrule
& {\arraybackslash\includegraphics[width=.7in]{figures/samples/6.png}} \\
User & Explain the humor of the image. \\
\\
\basename & The humor in the image arises from the unexpected and whimsical interaction between the two animals and the camera. The \textbf{squirrel}, typically a creature of the forest, is shown engaging with a human-made object, which is a \textbf{camera}. This anthropomorphism creates a playful and amusing scenario, as it is not common to see a squirrel with a camera. The \textbf{bird}, while not directly interacting with the camera, adds to the humor by being perched on the \textbf{tripod}, which is a human-made object, further blurring the lines between the natural and the artificial. The image plays on the idea of \textbf{animals being curious about human technology} and \textbf{the unexpected ways in which they might interact with it}. The humor is also enhanced by \textbf{the contrast between the natural setting and the human-made objects}, creating a surreal and entertaining scene. \\ 
\\
GPT-4V & The humor in this image comes from the role reversal and anthropomorphism on display. Typically, it's humans who photograph wildlife, but here, the \textbf{squirrel} is the one operating the \textbf{camera}, aiming it at the \textbf{bird}, as if it's about to take a picture. The bird, on the other hand, is posing like a subject of a photograph. This \textbf{unexpected switch}, along with \textbf{the attribution of human-like behavior to the animals}, creates a whimsical and amusing scene that deviates from the norm, which is the essence of humor. Additionally, the fact that the camera is set on top of a mushroom adds another layer of fantasy and playfulness to the image. \\
\\
LLaVA-v1.6-34B & The humor in this image comes from the anthropomorphism of the squirrel, which is a technique where human traits, emotions, or intentions are attributed to non-human entities. The \textbf{squirrel} is posed as if it is a \textbf{photographer}, holding a \textbf{camera} and seemingly \textbf{taking a picture of the bird}. This is amusing because it's a playful and imaginative scenario that suggests the squirrel is engaging in human-like behavior, which is not possible in reality. The juxtaposition of \textbf{a small, wild animal acting like a human photographer is whimsical and lighthearted}, evoking a sense of amusement and wonder. \\
 \\
LLaVA-v1.5-13B & The image features a \textbf{squirrel} standing on its hind legs and holding a camera, seemingly taking a picture of a \textbf{bird}. This scene is quite humorous as it portrays the squirrel as a photographer, which is an unusual and amusing sight. The bird, on the other hand, is perched on a \textbf{mushroom}, adding to the whimsical nature of the scene. The combination of the \textbf{squirrel's human-like behavior and the bird's presence} creates a light-hearted and entertaining image. \\
\toprule
\multicolumn{2}{l}{\textbf{Example 2: emotion detection }}  \\
\midrule
& {\arraybackslash\includegraphics[width=1in]{figures/samples/7.jpg}} \\
User & Based on the visual cues, what is the facial expression of the woman? \\
\\
\basename & The woman's facial expression can be described as \textbf{solemn and introspective}. Her eyes are slightly narrowed, and her mouth is closed in a neutral position, which often conveys a sense of \textbf{seriousness or deep thought}. The overall impression is one of \textbf{quiet contemplation or a moment of reflection}. \\ 
\\
GPT-4V & The woman in the image appears to have a \textbf{neutral or contemplative expression}. Her eyes are slightly downcast, and her mouth is closed in a relaxed manner, which does not convey a strong emotion. The overall impression is one of \textbf{calmness or pensiveness}. \\
\\
LLaVA-v1.6-34B & The woman in the image appears to have a \textbf{neutral to slightly serious facial expression}. Her eyebrows are slightly furrowed, and her mouth is closed, which could suggest a thoughtful or contemplative mood. The \textbf{white markings} on her face, which are often \textbf{associated with cultural or traditional significance}, add a unique and striking element to her appearance.\\
\\
LLaVA-v1.5-13B & The woman in the image has a \textbf{serious} facial expression, as she is looking directly at the camera. \\
\bottomrule
\end{tabular}
\caption{ Qualitative results of \shortname{3}. The bold words are annotated afterwards to highlight the key information.}
\label{tab:qualitative}
\end{table*}

% \begin{table*}[!ht]
% % \vspace{-10pt}
% \footnotesize
% \centering
% % \begin{tabular}{llcp{5cm}l}
% \begin{tabular}{m{1in}m{9cm}m{5cm}}
% \toprule
% \textbf{Prompt} & \textbf{\basename} & \textbf{LLaVA-V1.5-13B} \\
% \midrule
% {\arraybackslash\includegraphics[width=1in]{figures/samples/1.png}} & \multirow{2}{9cm}{
%  The humor in the image comes from the juxtaposition of the dog's relaxed posture and the common human experience of feeling lethargic or unenthusiastic on Mondays. The dog's laid-back demeanor, with its head resting on its paws and a seemingly contented expression, contrasts with the typical Monday morning rush and the associated stress. The text "Just Monday..." serves as a punchline, suggesting that the dog's state of restfulness is a humorous take on the human tendency to feel drained or unmotivated on the first day of the workweek. The image plays on the shared cultural experience of Monday blues, a term used to describe the feeling of dread that some people experience at the start of the workweek.} & \multirow{2}{5cm}{The image features a small dog lying on a hardwood floor.} \\ [100pt]
%  Explain the humor of the image. &\\ \hline
% \centering\arraybackslash\includegraphics[height=.7in]{figures/samples/4.png} & What is funny about this boy?
%  & The humor in this image arises from the visual pun created by the arrangement of the grapes. \textbf{The grapes are positioned in such a way that they resemble a cluster of balloons, with the stem acting as the string that the boy is holding}. The boy’s upward gaze and the way he is holding the stem suggest that \textbf{he is looking at the grapes as if they were floating balloons}, which is a playful and whimsical interpretation of the image. The simplicity of the line drawing adds to the comedic effect by allowing the viewer to fill in the details with their imagination, thus creating a light-hearted and amusing visual joke. \\ \hline
% \centering\arraybackslash\includegraphics[height=.7in]{figures/samples/2.png} & Can you give me a short introduction to this movie?
%  & The image appears to be from the movie “\textbf{The Godfather},” which is a landmark film in cinema history, directed by Francis Ford Coppola. The film is an adaptation of the novel of the same name by Mario Puzo. It is set in a post-World War II era and revolves around the fictional Corleone crime family. The central character is \textbf{Vito Corleone}, the patriarch of the family, played by Marlon Brando, who is seen here in a moment of strategic discussion with his consigliere, \textbf{Tom Hagen}, played by Robert Duvall. The film is renowned for its rich character development, \textbf{complex portrayal of organized crime}, and its \textbf{exploration of themes such as power, family, and corruption}. It is widely regarded as one of the greatest films in world cinema and has had a significant impact on the gangster film genre. \\ \hline
% \centering\arraybackslash\includegraphics[height=.7in]{figures/samples/3.jpg} & What is the model of the car?
%  & The model of the car is not explicitly stated in the image, but based on the distinctive design features such as the side air intakes, the shape of the headlights, and the overall body style, it resembles a McLaren MP4-12C, which is known for such design elements. The MP4-12C was the first model in the McLaren MP4-12C line, which is now known simply as the McLaren 650S and 720S series. To confirm the exact model, one would typically look for a badge or emblem on the car, which is not visible in this image, or refer to the vehicle identification number (VIN) if available. \\ \hline
% \centering\arraybackslash\includegraphics[height=.7in]{figures/samples/5.png} & What is unusual in the image?
%  & The unusual aspect of the image is the presence of \textbf{an individual using a manual clothes drying rack on the back of a moving yellow car}, which is \textbf{not a common sight in urban settings}. This juxtaposition of domestic activity and vehicular movement creates a striking and whimsical scene. \textbf{The contrast} between the \textbf{mundane task of laundry} and the \textbf{bustling city environment}, further emphasized by the passing taxi, adds to the \textbf{peculiarity of the situation}. It challenges the viewer’s expectations of what is typical in a city street and invites curiosity about the story behind this unusual choice of laundry day activity. \\
% \bottomrule
% \end{tabular}
% \caption{ Qualitative results of \shortname{13}. The bold words are annotated afterwards to highlight the key information.}
% \label{tab:qualitative}
% \end{table*}

We provide two examples and compare the generation results between ALLaVA and other SOTA models, including GPT-4V, LLaVA-v1.5-13B and LLaVA-v1.6-13B\footnote{Results are obtained from \url{https://llava.hliu.cc/} on Feb. 9th, 2024.}.
Example 1 tests the model ability on humor comprehension. All four models are able to generate satisfactory descriptions on the image, capturing the posture of the squirrel and the bird and identifying their respective roles, which adds humor to the image.
Example 2 probes the ability to detect emotion. ALLaVA, GPT-4V and LLaVA-v1.6-34B have consistent judgement on the woman's facial expression and her underlying emotion. However, LLaVA-v1.5-13B only has a superficial description and states that she is looking at the camera, which she is not.

In these two examples, ALLaVA, with only 3B parameters, is able to achieve comparable performance with much larger models, demonstrating its superior reasoning ability gained from our high-quality training set.


\subsection{Analysis}
\paragraph{Ablation on Data}

\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{cc  c c c }
\toprule
PT w/ \ptname & FT w/ \ftname & MM-Vet & MME & GQA \\ \midrule
\xmark & \xmark & 25.8 & 1489.9 & 44.0  \\ 
\xmark & \cmark & 12.1 & 1199.8 & 39.0  \\
\cmark & \xmark & 30.0 & 1582.1 & 47.7 \\ 
\cmark & \cmark & \textbf{32.2} & \textbf{1623.2} &  \textbf{50.0} \\
\bottomrule
\end{tabular}
\caption{Ablation of using our data on three benchmarks. PT: pretraining, or vision-language alignment. FT: finetuning, or visual instruction tuning.}
\label{tab:ablation_cap_inst}
\end{table}

Table~\ref{tab:ablation_cap_inst} details the results of training the model with or without our data at each stage.
The baseline result (line 1) is obtained by solely using ShareGPT4V for alignment, and llava\_instruct\_657K for instruction tuning.
Adding solely ALLaVA-Instruct-4V (line 2) performs even worse than using either of our data (line 1), but adding both (line 4) performs better than adding solely ALLaVA-Caption-4V (line 3). This indicates that one cannot perform large scale visual instruction tuning on an insufficiently aligned model.
Involving both of our datasets (line 4) significantly improves the model performance on these three benchmarks, manifesting the effectiveness of our datasets.


% However, there is relatively small improvement when adding \ftname to a well-aligned model (line 2 to line 3). This can be attributed to that these benchmarks contain only \textit{simple} instructions, which may have limited improvement using \textit{complex} instructions.
% Overall, we demonstrate that both \ptname and \ftname are effective in significantly improving the performance of LVLMs.


% \begin{table}[t]
% \centering
% \begin{tabular}{c|c c c | c c c }
% \toprule
% LM & laion\_cap & vflan\_cap & sharegpt4v & MM-Vet & MMMU$^{val}$ & MB \\ \midrule
% - & \xmark & \xmark & \cmark \\
% - & \cmark & \xmark & \cmark \\
% - & \xmark & \cmark & \cmark \\
% - & \cmark & \cmark & \cmark \\
% \bottomrule
% \end{tabular}
% \caption{Effect of our caption data on three benchmarks.}
% \label{tab:my_label}
% \end{table}


% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{l c c c c }
% \toprule
% Name (LM backbone)  & Vicuna-80 & MM-VET &MME & GQA \\ \midrule
% ALLaVA (Qwen-1.8B) & 40.0 & 28.3 & 1467.0 & 48.7 \\
% ALLaVA (StableLM-2-1.6B) & 38.1 & 32.7 & 1539.1 & 49.9 \\
% \textbf{ALLaVA (Phi2-2.7B) } & \textbf{48.8} & \textbf{33.2} & \textbf{1623.2} & \textbf{50.0}\\
% \bottomrule
% \end{tabular}
% \caption{Comparison of different LLM backbones. In the default setting, we use Phi2-2.7B as the LM backbone as it performs the best. }
% \label{tab:ablation_lm}
% \end{table}




% \paragraph{Choice of LM Backbones}


% %%%%%%%%%%%%%%%%%%%%% LM Backbone %%%%%%%%%%%%%%%%%%%%%
% \begin{table}[t]
% \centering
% \footnotesize
% \resizebox{\textwidth}{!}{
% \setlength{\tabcolsep}{2pt}
% \begin{tabular}{ l  c c c c c c c c c c c c c c c c c}
% % \begin{tabular}{ l  l  c  p{.4cm} p{.9cm} c p{1.0cm} p{.6cm} p{.5cm} p{.4cm} p{.9cm}  c c  c }
% \toprule
% \vspace{2pt} 
% Model & Vicuna-80 & GQA & HallB & MV & MM-Vet & MMB-en & MMB-cn & MME-P & MME-C & MMMU\(^{val}\) & MMVP  & SQA$^I$ & SEED\(_{img}^{v1}\) & VQA$^T$  & LLaVA\(^{W}\) & \textbf{MB} & TS \\
% \midrule
% ALLaVA-Phi2 & 49.4 & 48.8 & 24.8 & 27.4 & 32.2 & 64.0 & 40.8 & 1316.2 & 301.8 & 35.3 & 36.0 & 67.6 & 65.2 & 49.5 & 69.4 & - & 632.0\\
% ALLaVA-StableLM2  & 38.8 & 49.8 & 25.3 & 27.7 & 31.7 & 64.6 & 49.8 & 1311.7 & 257.9 & 33.3 & 34.0 & 64.7 & 65.7 & 51.7 & 72.0 & 39.3 & 655.2\\
% ALLaVA-Phi3 & \textbf{56.9} & 52.2 & \textbf{48.1} & \textbf{32.9} & \textbf{37.8} & 68.1 & \textbf{55.3} & 1382.3 & \textbf{347.1} & \textbf{41.1} & 32.7 & 64.0 & 69.0 & 53.0 & 68.5 & \textbf{54.8} & \textbf{667.8}\\
% \rowcolor{lightgray}
% ALLaVA-LLaMA3 & 60.6 & 51.1 & 39.0 & 27.3 & 35.4 & 70.7 & 64.6 & 1379.4 & 341.4 & 34.3 & 29.3 & 70.0 & 70.0 & 57.8 & 76.1 & 54.3 & 642.3\\
% \bottomrule
% \end{tabular}
% }
% % \vspace{-1mm}
% \caption{
% Comparison of different LLM backbones. In the default setting, we use Phi3-mini as the LM backbone as it performs the best.
% }
% \label{tab:ablation_lm}
% \end{table}
% %%%%%%%%%%%%%%%%%%%%% LM Backbone %%%%%%%%%%%%%%%%%%%%%


% %%%%%%%%%%%%%%%%%%%%% LVLMs %%%%%%%%%%%%%%%%%%%%%
% \begin{table}[ht!]
% \centering
% \footnotesize
% \resizebox{\textwidth}{!}{
% \setlength{\tabcolsep}{2pt}
% \begin{tabular}{ l c c c c c c c c c c c c c c c c c}
% % \begin{tabular}{ l  l  c  p{.4cm} p{.9cm} c p{1.0cm} p{.6cm} p{.5cm} p{.4cm} p{.9cm}  c c  c }
% \toprule
% \vspace{2pt} 
% Model & Vicuna-80 & GQA & HallB & MV & MM-Vet & MMB-en & MMB-cn & MME-P & MME-C & \textbf{MMMU\(^{val}\)} & \textbf{MMVP}  & SQA$^I$ & SEED\(_{img}^{v1}\) & \textbf{VQA$^T$ } & \textbf{LLaVA\(^{W}\)} & MB & \textbf{TS} \\
% \midrule
% MobileVLM-v2* &  5.0* & 61.1 & 30.8* & 28.3* & 26.1* & 63.2 & 43.2* & 1440.5 & 261.8* & 30.8* & 18.7* & 70.0 & 64.5* & 57.5 & 53.2* & 15.7* & 541.0*\\
% MobileVLM-v2-ALLaVA  & 3.1 & 59.9 & 29.1 & 27.9 & 36.1 & 62.7 & 44.0 & 1440.6 & 273.6 & 33.3 & 25.3 & 71.6 & 64.6 & 58.3 & 64.6 & 33.1 & 631.3\\
% Mipha-3B  & 16.2* & 63.9 & 34.3* & 27.8* & 33.5* & 69.7 & 42.9* & 1488.9 & 285.0* & 35.8* & 32.0* & 70.9 & 71.2* & 56.6 & 64.7* & 23.1* & 619.0*\\
% Mipha-3B-ALLaVA  & 0.0 & 63.3 & 31.8 & 33.0 & 23.2 & 72.2 & 47.6 & 1459.1 & 313.2 & 39.0 & 45.3 & 71.8 & 71.7 & 58.0 & 79.5 & 8.6 & 708.4\\
% \bottomrule
% \end{tabular}
% }
% % \vspace{-1mm}
% \caption{
% {\guiming{consider making it a chart}}
% Ablation on existing LVLMs. Both MobileVLM-v2\needcite and Mipha\needcite adopts the PT-FT training paradigm. We add ALLaVA-Caption-4V and ALLaVA-Instruct-4V to PT and FT, respectively.
% }
% \label{tab:ablation_lvlms}
% \end{table}
% %%%%%%%%%%%%%%%%%%%%% LVLMs %%%%%%%%%%%%%%%%%%%%%


% Table~\ref{tab:ablation_lm} details the results of using different LM backbones.
% The language performance of using Phi2-2.7B after multimodal training is significantly better than using Qwen-1.8B~\citep{bai2023qwen} and StableLM-2-1.6B~\citep{StableLM-2-1.6B}. On multimodal benchmarks, using Phi2-2.7B outperforms Qwen-1.8B by a larger margin than StableLM-2-1.6B. This result suggests the potential of adopting StableLM for multimodal training.


% \paragraph{Ablation on Existing LVLMs}
% Results in Table~\ref{tab:ablation_lvlms}




